Recovering PCA from Hybrid-$(\ell_1,\ell_2)$ Sparse Sampling of Data Elements

This paper addresses how well we can recover a data matrix when only given a few of its elements. We present a randomized algorithm that element-wise sparsifies the data, retaining only a few its elements. Our new algorithm independently samples the data using sampling probabilities that depend on both the squares ($\ell_2$ sampling) and absolute values ($\ell_1$ sampling) of the entries. We prove that the hybrid algorithm recovers a near-PCA reconstruction of the data from a sublinear sample-size: hybrid-($\ell_1,\ell_2$) inherits the $\ell_2$-ability to sample the important elements as well as the regularization properties of $\ell_1$ sampling, and gives strictly better performance than either $\ell_1$ or $\ell_2$ on their own. We also give a one-pass version of our algorithm and show experiments to corroborate the theory.

==> supplementary_exp2.tex <==
%=============================================================
\subsection{Supplementary Experiments}
%
%
% ============================================
\remove{
\begin{figure}[!h]
\centering
	\includegraphics[height=3.2cm,width=5.6cm]{surrogate_synth_A10.eps}
%
	\includegraphics[height=3.2cm,width=5.6cm]{surrogate_digit.eps}
%
\caption{Approximation quality of $\tilde{\matA}_k$ as a surrogate for $\matA_k$: hybrid-$(\ell_1,\ell_2)$ sampling, for various $\alpha$ and two different $s$, are shown. Top and bottom datasets are ordered as $\matA 0.1$ and Digit. $x$-axis is $\alpha$, and $y$-axis plots ${\FNorm{\matA_k - \tilde{\matA}_k}}/{\FNorm{\matA_k}}$. We set $k=5$ for $\matA0.1$, and $k=3$ for Digit data. $y$-values are in log$_2$ scale such that larger negative values indicate better quality.}
\label{fig:surogate_approx}
\end{figure}
%
}%
% ============================================
\iffalse %  =========== COMMENTED OUT =================
\subsubsection{Iterative Estimate of $\alpha^*$}
%
We compare the quality of Algorithm \ref{alg:alg_iterative_alpha} producing an iterative estimate of $\alpha^*$ using one pass over the elements of data using $O(s)$ memory. Figure \ref{fig:compress_approx} plots approximation quality of the sparse sketches $\tilde{\matA}$ produced from the datasets for various $\alpha$ using different sample sizes. These results are generated without any restriction of size of memory or number of pass over the elements of the datasets. Table \ref{fig:alpha_tilde} lists $\tilde{\alpha}$, the estimated $\alpha^*$, for some of the datasets, for two choices of $s$ using 10 iterations. 
%
% ============================================
%\begin{figure}[!h]
%\centering
%%	\includegraphics[scale=0.16]{Synthetic_k_5_compress_spectral_noisy05_plot.eps}
%%	\includegraphics[height=3.0cm,width=5.2cm]{Synthetic_k_5_compress_spectral_noisy05_plot.eps}
%%	\includegraphics[height=2.5cm,width=4.6cm]{Synthetic_k_5_col_approx_spectral_noisy05_plot.eps}
%%	\includegraphics[height=2.5cm,width=4.5cm]{Synthetic_k_5_row_approx_spectral_noisy05_plot.eps}
%%
%	\includegraphics[height=3.0cm,width=5.2cm]{Synthetic_k_5_compress_spectral_noisy10_plot.eps}
%%	\includegraphics[height=2.5cm,width=4.6cm]{Synthetic_k_5_col_approx_spectral_noisy10_plot.eps}
%%	\includegraphics[height=2.5cm,width=4.5cm]{Synthetic_k_5_row_approx_spectral_noisy10_plot.eps}
%%
%\caption{Approximation quality of $\tilde{\matA}$ for data $\matA0.10$: hybrid-$(\ell_1,\ell_2)$ sampling for various $\alpha$ and three different $s$ are shown. $x$-axis is various values of $\alpha$, and $y$-axis denotes ${\TNorm{\matA - \tilde{\matA}}}/{\TNorm{\matA}}$. We set $k=5$ for this dataset. $y$-values are in log$_2$ scale such that larger negative values indicating better quality.} 
%\end{figure}
%
%
% ============================================
%
%  ===============================================
%\begin{table}[!h]
%\begin{center}
%    \begin{tabular}{|  l | l | l | l | l | l | l | l | }
%   \hline
% Data & $\matA0.05$ & $\matA0.1$ & TechTC1 & TechTC2& TechTC3 & TechTC4 & Digit   \\ \hline \hline  
%$\alpha^*$, $\epsilon=0.05$ & 0.62 & 0.63 & \qquad 1 & \qquad 1 & \qquad 1 & \qquad 1 & 0.20 \\\hline 
%$\alpha^*$, $\epsilon=0.75$ & 0.69 & 0.70 & \qquad 1 & \qquad 1 & \qquad 1 & \qquad 1 & 0.74 \\\hline 
%    \end{tabular}
%\caption{$\alpha^*$ for various data sets ($\epsilon$ is given relative-error accuracy)}
%\label{fig:alpha_opt}
%\end{center}
%\end{table}
%  ===============================================
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  l | l | l |}
   \hline
 \qquad \quad & $\frac{s}{k\cdot (m+n)} = 2$ & $\frac{s}{k\cdot (m+n)} = 3$   \\ \hline \hline  
$\matA_{0.05}, k=5$ & \qquad 0.54 & \qquad 0.48 \\ \hline
$\matA_{0.1}, k=5$ & \qquad 0.55 & \qquad 0.5 \\ \hline
%TechTC1, $k=2$ &  \qquad 0.93 & \qquad  1 \\ \hline
%TechTC2, $k=2$ &  \qquad 1 & \qquad 1 \\ \hline
%TechTC3, $k=2$ &  \qquad 0.97 & \qquad 0.85 \\ \hline
%TechTC4, $k=2$ &  \qquad 0.79 & \qquad 1 \\ \hline
Digit, $k=3$ & \qquad 0.69 & \qquad 0.89 \\ \hline
Stock, $k=1$ & \qquad 1 & \qquad 1 \\ \hline
   \end{tabular}
\caption{Values of $\tilde{\alpha}$ (estimated $\alpha^*$ using Algorithm \ref{alg:alg_iterative_alpha}) for various data sets using one pass over the elements of data and $O(s)$ memory. We use $\epsilon=0.05$, $\delta=0.1$.}
\label{fig:alpha_tilde}
\end{center}
\end{table}
\fi %  =========== END OF COMMENTED OUT =================
% ============================================
\iffalse
\subsubsection{Fast Approximation of PCA}
% ============================================
Here we show the visual quality of the projected data $\matA_{0.1}$ onto the top five principal components (exact and approximate). Figure \ref{fig:PCA_synth} shows the heatmap of the approximation. 
% ============================================
\begin{figure}[!h]
\centering
	\includegraphics[height=2.8cm,width=8.2cm]{PCA_approx_synth_rank5_heatmap2.png}
%
\caption{
Approximation quality of fast PCA (Algorithm \ref{alg:alg_approx_PCA}) for data $\matA_{0.1}$. Visualization of projected data onto top five PCs. Left image  shows the projected actual data onto the exact PCs. Middle image is the projection of actual data onto approximate PCs (of sampled data). We observe a similar quality for $\matA_G$. Right image shows the projected sparsified data onto approximate PCs (of sampled data). We use only 6\% of all elements to produce the sparse sketch.
}
\label{fig:PCA_synth}
\end{figure}
%
\fi
%
%
\iffalse % ============ COMMENTED OUT ===========
% ============================================
\subsubsection{Comparison with Leverage Score Sampling}
%  ===============================================
Here we compare the sparsification quality of rank-truncated $\matA).1$ using $k=5$ (Table \ref{fig:lev_comp_synth}). We observe that rank-truncated $\matA_{0.1}$ is effectively a sparse matrix. Our optimal hyrbid-$(\ell_1,\ell_2)$ probabilities are better aligned with the structure of the data, resulting in superior approximation quality.
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  l | l | l |}
   \hline
\qquad \quad & Hybrid-$(\ell_1,\ell_2)$ & \quad $p_{lev}$    \\ \hline \hline  
$\frac{s}{k(m+n)}=3$ & \qquad  25\% & \quad  80\% \\ \hline
$\frac{s}{k(m+n)}=5$ & \qquad 21\% \quad & \quad 62\% \\ \hline
   \end{tabular}
\caption{
Sparsification of rank-truncated $\matA_{0.1}$ matrix ($k=5$). We compare the quality of $\TsNorm{\matA - \tilde{\matA}}/\TsNorm{\matA}$ for hybrid-$(\ell_1,\ell_2)$ sampling (average $\alpha^*  = 0.71$ using $\epsilon=0.05, \delta=0.1$) and leverage score sampling using two sample sizes.
}
\label{fig:lev_comp_synth}
\end{center}
\end{table}
\fi %  % ============ END OF COMMENTED OUT ===========
\remove{ % ============ COMMENTED OUT ===========
%
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  l | l | l |}
   \hline
\qquad \quad & Hybrid-$(\ell_1,\ell_2)$ & \quad Leverage    \\ \hline \hline  
$\frac{s}{k(m+n)}=3$ & \qquad  44\% & \qquad  61\% \\ \hline
$\frac{s}{k(m+n)}=5$ & \qquad 34\% \quad & \qquad 47\% \\ \hline
   \end{tabular}
\caption{
Sparsification of rank-truncated Digit matrix ($k=3$). We compare the quality of $\TNorm{\matA - \tilde{\matA}}/\TNorm{\matA}$ for hybrid-$(\ell_1,\ell_2)$ sampling ($\alpha^*  = 0.2$ using $\epsilon=0.05, \delta=0.1$) and leverage score sampling using two sample sizes.
}
\label{fig:lev_comp_digit}
\end{center}
\end{table}
} % ============ END OF COMMENTED OUT ===========
% ============================================
\remove{ % ============ COMMENTED OUT ===========
\begin{figure}[!h]
\centering
	\includegraphics[height=3.6cm,width=5.2cm]{lev_vs_hybrid_Chen_s3.eps}
%
	\includegraphics[height=3.6cm,width=5.2cm]{lev_vs_hybrid_Chen_s5.eps}
%
\caption{
Sparsification quality $\TNorm{\matA_{pow} - \tilde{\matA}_{pow}}/\TNorm{\matA_{pow}}$  of low-rank `power-law' matrix $\matA_{pow}$ ($k=5$). We compare the quality of hybrid-$(\ell_1,\ell_2)$ sampling and leverage score sampling using two sample sizes: 
$s = 3\cdot k(m+n)$ (\textit{top figure}), and $s = 5\cdot k(m+n)$ (\textit{bottom figure}) .
We note (average) $\alpha^*$ of hybrid-$(\ell_1,\ell_2)$ distribution for data $\matA_{pow}$ using $\epsilon=0.05, \delta=0.1$. For $\gamma=0.5, 0.8, 1.0$, we have $\alpha^* = 0.11, 0.72, 0.8$, respectively. 
}
\label{fig:lev_comp_Chen}
\end{figure}
%
}
%
% ============================================

